Robust causal structure learning with some hidden variables

We introduce a new method to estimate the Markov equivalence class of a directed acyclic graph (DAG) in the presence of hidden variables, in settings where the underlying DAG among the observed variables is sparse, and there are a few hidden variables that have a direct effect on many of the observed ones. Building on the so-called low rank plus sparse framework, we suggest a two-stage approach which first removes the effect of the hidden variables, and then estimates the Markov equivalence class of the underlying DAG under the assumption that there are no remaining hidden variables. This approach is consistent in certain high-dimensional regimes and performs favourably when compared to the state of the art, both in terms of graphical structure recovery and total causal effect estimation.

==> Sections/Identifiability.tex <==
The high-dimensional behaviour of the Low-Rank plus Sparse decomposition (LRpS henceforth) and the GES algorithm has been studied in the literature \citep{ChandrasekaranParriloWillsky12, NandyHauserMaathuis16}, 
and rely on this body of work to study the theoretical properties of our approach.
While the technical details underpinning the LRpS estimator are beyond the scope of this paper, 
it is useful to get an intuition for when our estimator is expected to produce meaningful results.
For that reason, we start by recalling a few key properties of LRpS. We then state our main result: the high-dimensional consistency of LRpS+GES.

\subsection{Key Properties of LRpS}
\label{identifiability}
Earlier, it was mentioned that while the problem
under study is fundamentally misspecified, it admits a unique solution when 
$K_O^\ast$ is sparse and $L^\ast$ is low-rank.
However, the concepts of ``sparsity'' and ``rank'' are not precise enough in this context. 
For example, consider a matrix with a single entry: it is
both sparse and low-rank, so that there is no unique way of writing it as the sum of a sparse and a low-rank matrix.
\cite{ChandrasekaranEtAl11} and \cite{CandesEtAl11} introduced two quantities which are better 
suited to the study of the identifiability of \eqref{lrps_estimator} (we refer the reader to 
\cite{ChandrasekaranEtAl11} for precise mathematical definitions): 
\begin{itemize}
    \item $\xi(L^\ast)$: a small value of $\xi(L^\ast)$ guarantees that no single latent variable will have
    an effect on only a small number of the observed variables. It is related to the concept of \emph{incoherence} found 
    in \cite{CandesEtAl11}. This is useful because $\xi$ is not easy to compute in general while
    the incoherence of some arbitrary matrix $M$ ($inc(M)$)
    is easily calculated and satisfies $inc(M) \leq \xi(M) \leq 2inc(M)$.
    \item $\mu(K_O^\ast)$ quantifies the diffusivity of $K_O^\ast$'s spectrum. Matrices that have a small $\mu$
        have few non-zero entries per row/column. Thus, $\mu(K_O^\ast)$ is also related to the degree of $K_O^\ast$ (\emph{i.e.} maximum number of non-zero entries in any given row/column). 
\end{itemize}

An important condition for identifiability can be expressed in terms of $\xi, \mu$ by requiring 
that their product be small enough ($\xi(L^\ast) \mu(K_O^\ast) \leq \frac{1}{6}C^2$) 
and that the tuning parameter $\gamma$ be chosen within a given range 
($\gamma \in \left[\frac{3\xi(L^\ast)}{{C}}, \frac{C}{2\mu(K_O^\ast)}\right]$),
for some constant ${C}$ which depends on the Fisher information matrix. 
This means that there must be few latent variables acting on many observed ones and that $K_O^\ast$ must
have bounded degree. %Interestingly, there are natural classes of matrices satisfying this condition.
%Of particular interest to us is the regime where the degree of $K_O^\ast$ is of the form $K_O^\ast = \mathcal{O}(\log(p)^d)$
%and the number of latent variables $h$ is also allowed to grow with $p$: $h = \mathcal{O}(\frac{p}{\log (p)^{2d}})$ (see \citep[\S4.2]%{ChandrasekaranParriloWillsky12}).

